Large Magellanic Cloud Near-Infrared Synoptic Survey. V. Period-Luminosity Relations of Miras

We study the near-infrared properties of 690 Mira candidates in the central region of the Large Magellanic Cloud, based on time-series observations at JHKs. We use densely-sampled I-band observations from the OGLE project to generate template light curves in the near infrared and derive robust mean magnitudes at those wavelengths. We obtain near-infrared Period-Luminosity relations for Oxygen-rich Miras with a scatter as low as 0.12 mag at Ks. We study the Period-Luminosity-Color relations and the color excesses of Carbon-rich Miras, which show evidence for a substantially different reddening law.

==> tab01.tex <==
\begin{center}
\begin{deluxetable*}{lrrrrrr}[!t]
\tablecaption{Predictors and Coefficients for the Regression Model\label{tbl_lmp}}
\tablewidth{\textwidth}
\tabletypesize{\footnotesize}
\tablehead{
\colhead{Predictor}  & \multicolumn6c{Regression Coefficients} \\ \cline{2-7}
& \multicolumn3c{O-rich} & \multicolumn3c{C-rich} \\
 \multicolumn1r{$(I - )$} & \colhead{$J$} & \colhead{$H$} & \colhead{$K_s$} & \colhead{$J$} & \colhead{$H$} & \colhead{$K_s$}
}
\startdata
              $\ast I_\mathrm{abs}$ &  7.9e-01 &  7.4e-01 &  7.3e-01 &  3.4e-01 &  3.7e-01 &  4.4e-01\\
            $\ast I_\mathrm{abs}^2$ &       NA &       NA &       NA & -2.0e-03 & -1.1e-02 & -3.5e-03\\
 $\ast F = 10^{-0.4I_\mathrm{abs}}$ &  2.1e-03 &       NA &       NA &       NA &       NA & -4.8e-04\\
                         $\ast F^2$ &       NA &  1.4e-05 &  8.9e-06 &  2.8e-06 &       NA &       NA\\
                         $\ast F^3$ & -1.2e-08 & -3.7e-08 & -2.0e-08 &       NA &       NA &       NA\\
                     $\ast F^{0.5}$ &       NA &       NA &       NA &       NA &       NA & -4.5e-02\\
              $\ast \cos(2\pi\phi)$ &       NA & -8.4e-03 & -4.0e-02 &  6.1e-02 &  4.6e-02 &  4.3e-02\\
              $\ast \sin(2\pi\phi)$ &  1.9e-01 &  2.0e-01 &  2.1e-01 &  7.2e-02 &  8.3e-02 &  7.7e-02\\
              $\ast \cos(4\pi\phi)$ &  1.4e-02 &  1.1e-02 &  1.5e-02 & -3.5e-03 & -1.9e-03 &       NA\\
              $\ast \sin(4\pi\phi)$ &  9.4e-03 &  1.6e-02 &  1.8e-02 &  1.7e-02 &  1.8e-02 &  1.8e-02\\
              $\ast \cos(6\pi\phi)$ &  1.7e-02 &  7.7e-03 &  7.7e-03 &  5.2e-03 &  6.6e-03 &       NA\\
              $\ast \sin(6\pi\phi)$ &       NA &       NA &       NA & -4.8e-03 & -9.0e-03 & -1.3e-02\\
                                $P$ & -7.7e-02 &  1.9e-02 &  3.4e-02 &  2.5e-03 &  5.4e-03 &  5.4e-03\\
                           $\log P$ &  6.3e+03 & -3.2e+03 & -5.5e+03 &       NA & -2.6e+01 & -3.3e+01\\
                          $\log^2P$ & -1.1e+03 &  4.8e+02 &  8.4e+02 &       NA &       NA &       NA\\
                          $\log^3P$ &  1.1e+02 & -4.5e+01 & -7.9e+01 &       NA &       NA &       NA\\
                      $\log^{0.5}P$ & -9.5e+03 &  5.0e+03 &  8.7e+03 &       NA &  7.7e+01 &  1.0e+02\\
                              $J-H$ & -5.6e-01 &  3.9e-01 &  3.5e-01 & -3.5e-01 &  4.8e-01 &  3.2e-01\\
                              $H-K$ & -5.4e-01 & -4.8e-01 &  4.1e-01 &       NA & -2.4e-01 &  3.9e-01\\
                              $A_I$ &  7.9e-03 &  1.7e-02 &  1.7e-02 &  5.0e-02 &  7.4e-02 &  1.0e-01\\
                          Intercept &  4.2e+03 & -2.3e+03 & -4.0e+03 &  2.7e+00 & -5.4e+01 & -7.3e+01\\
\hline
                     $\sigma$ [mag] &     0.12 &     0.12 &     0.12 &     0.12 &     0.13 &     0.15\\
\enddata
\tablecomments{Predictors beginning with $\ast$ indicates time-dependent quantities. NA indicates predictors that were rejected by the LASSO regularization.}
\end{deluxetable*}
\end{center}

